Variations on the Sensitivity Conjecture

We present a selection of known as well as new variants of the Sensitivity Conjecture and point out some weaker versions that are also open.

==> logrank_gap.tex <==
%\subsection*{A Quadratic Gap between $D_\oplus(f)$ and $s(f)$}

%Next we present a quadratic gap between $D_\oplus(f)$ and $s(f)$. 

%\begin{defn}
%The \emph{mod $2$ degree} of a Boolean funtion $f$, denoted by $\deg_\oplus (f)$, is the degree
%of the (unique) multilinear polynomial over $\mathbb{F}_2$ (the field of two elements)
%that represents $f.$
%\end{defn}
%It is easy to check that $\deg_\oplus(f) \leq D_\oplus(f).$ Moreover, the following holds:

%\begin{lem}[Bernasconi and Codenotti~\cite{bc}, Lemma~3]
%\label{bc_lemma}
%For every Boolean \\ function $f$, $\deg_\oplus(f) \leq \log \rank(f(x \oplus y)).$
%\end{lem}

%\begin{lem}[Rivest and Vuillemin~\cite{rv}]
%\label{rv_lemma}
%If $f$ is a transitive Boolean function on $n = 2^k$ variables
%such that $f({\bf 0}) \neq f({\bf 1})$, then $\deg_\oplus(f) = n.$  
%\end{lem}

%Consider the Boolean function $f({\bf x})=\bigwedge_{i=1}^{2^k} \bigvee_{j=1}^{2^k} x_{ij},$ on  
%$n=2^{2k}$ variables. It is easy to see that the OR and AND functions are of full mod $2$ degree; hence, $n= \deg_\oplus(f)\leq D_\oplus(f),$ by Lemma~\ref{bc_lemma}. The gap follows since $s(f) = 2^k=\sqrt n$. 

